Collaborative Decoding of Interleaved Reed-Solomon Codes and Concatenated Code Designs

Interleaved Reed-Solomon codes are applied in numerous data processing, data transmission, and data storage systems. They are generated by interleaving several codewords of ordinary Reed-Solomon codes. Usually, these codewords are decoded independently by classical algebraic decoding methods. However, by collaborative algebraic decoding approaches, such interleaved schemes allow the correction of error patterns beyond half the minimum distance, provided that the errors in the received signal occur in bursts. In this work, collaborative decoding of interleaved Reed-Solomon codes by multi-sequence shift-register synthesis is considered and analyzed. Based on the framework of interleaved Reed-Solomon codes, concatenated code designs are investigated, which are obtained by interleaving several Reed-Solomon codes, and concatenating them with an inner block code.

==> defs.tex <==
\DeclareMathAlphabet{\mathbcal}{OMS}{cmsy}{b}{n}

\DeclareMathOperator{\de2}{d^2_{\mathcal{E}}}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\wt}{wt}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\neras}{\mathcal{N}}
\DeclareMathOperator{\erfc}{erfc}
\DeclareMathOperator{\dist}{dist}
\DeclareMathOperator{\dB}{dB}

\newcommand{\wbar}[1]{\setbox0=\hbox{\ensuremath{#1}}%
  \dimen0=\ht0\advance\dimen0 by0.2ex%
  \dimen3=\ht0\multiply\dimen3 by17\divide\dimen3 by100%
  \dimen1=\wd0\advance\dimen1 by-\dimen3\advance\dimen1 by-0.08em%
  \dimen2=\dimen1\advance\dimen2 by-0.04em%
  \ensuremath{#1}%
  \kern-\dimen1\hbox{\rule[\dimen0]{\dimen2}{0.47pt}}%
} 

\newcommand{\eras}{\ensuremath{\varepsilon}}

\newcommand{\set}[1]{\ensuremath{#1}}
\newcommand{\abs}[1]{\ensuremath{\left|#1\right|}}
\newcommand{\vect}[1]{\ensuremath{\boldsymbol{#1}}}
\newcommand{\fvect}[1]{\ensuremath{\boldsymbol{\mathsf{#1}}}}
\newcommand{\mat}[1]{\ensuremath{\boldsymbol{#1}}}
\newcommand{\submatr}[3]{\ensuremath{left.\boldsymbol{#1}\right|_{#2}^{#3}}}

\newcommand{\card}[1]{\ensuremath{\left|{#1}\right|}}
\newcommand{\code}{\ensuremath{\mathcal{C}}}
\newcommand{\codeo}{\ensuremath{\mathcal{A}}}
\newcommand{\codei}{\ensuremath{\mathcal{B}}}
\newcommand{\codeg}{\ensuremath{\mathcal{K}}}
\newcommand{\codet}{\ensuremath{\mathcal{L}}}
%\newcommand{\rscode}{\ensuremath{\mathcal{C}_{\text{RS}}}}
\newcommand{\rscode}{\ensuremath{\mathcal{A}}}
\newcommand{\irscode}{\ensuremath{\boldsymbol{\mathcal{A}}}}

\newcommand{\Mset}{\ensuremath{\mathcal{S}}}

\newcommand{\BCH}{\ensuremath{\text{BCH}}}
\newcommand{\G}[1]{\ensuremath{\mathcal{G}}\left({#1}\right)}
\newcommand{\RM}[1]{\ensuremath{\mathcal{RM}}\left({#1}\right)}
\newcommand{\RS}[1]{\ensuremath{\mathcal{RS}\left({#1}\right)}}
\newcommand{\IRS}[1]{\ensuremath{\mathcal{IRS}({#1})}}

\newcommand{\F}[1]{\ensuremath{\mathbb{F}}_{#1}}
\newcommand{\E}{\ensuremath{\mathbb{E}}}
\newcommand{\CE}{\ensuremath{\mathcal{E}}}
\newcommand{\ce}{\ensuremath{\epsilon}}
\newcommand{\FF}[2]{\ensuremath{\mathbb{F}}_{#1}^{#2}}
\newcommand{\GF}[1]{\ensuremath{\text{GF}}\left({#1}\right)}

\newcommand{\intersec}{\ensuremath{\mathcal{D}}}

\newcommand{\FT}[1]{\ensuremath{\mathscr{F}\left({#1}\right)}}
\newcommand{\IFT}[1]{\ensuremath{\mathscr{F}^{-1}\left({#1}\right)}}

\newcommand{\Et}[1]{\ensuremath{\mathcal{E}_t\left({#1}\right)}}

\newcommand{\alg}[1]{\textsf{{#1}}}
\newcommand{\algcomment}[1]{\textsf{\footnotesize/$\ast$\ {#1}$\ \ast$/}}

\newcommand{\Set}[1]{\ensuremath{\left\{{#1}\right\}}}
\newcommand{\SetL}[1]{\ensuremath{\mathcal{#1}}}

\newcommand{\SSeq}{\SetL{S}}
\newcommand{\SSeqh}[1]{\SetL{S}^{({#1})}}
\newcommand{\Seq}[3]{\ensuremath{\{{#1}\}_{#2}^{#3}}}

\newcommand{\avg}[1]{\ensuremath{\bar{#1}}}
\newcommand{\maxi}[1]{\ensuremath{\widehat{#1}}}

\newcommand{\tg}{\ensuremath{t_\mathrm{g}}}
\newcommand{\tm}{\ensuremath{t_\mathrm{max}}}
\newcommand{\tr}{\ensuremath{\vartheta}}

\newcommand{\transp}[1]{\ensuremath{{#1}^\mathsf{T}}}

\newcommand{\pwi}{\ensuremath{p_{w}}}
\newcommand{\pwilb}{\ensuremath{\underline{p}_{w}}}
\newcommand{\pwiub}{\ensuremath{\overline{p}_{w}}}
\newcommand{\psy}{\ensuremath{p_\mathrm{s}}}
\newcommand{\psylb}{\ensuremath{\underline{p}_\mathrm{s}}}
\newcommand{\psyub}{\ensuremath{\overline{p}_\mathrm{s}}}
\newcommand{\pwoi}{\ensuremath{P_{w}^{\mathrm{i}}}}
\newcommand{\pwoc}{\ensuremath{P_{w}^{\mathrm{c}}}}
\newcommand{\pwo}{\ensuremath{P_{w}}}
\newcommand{\pwib}{\ensuremath{\hat{p}_{w}}}

\newcommand{\pwnc}[1]{\ensuremath{P_{e}^{\mathrm{i}}\left({#1}\right)}}
\newcommand{\pwc}[1]{\ensuremath{P_{c}^{\mathrm{i}}\left({#1}\right)}}
\newcommand{\pwnclb}[1]
{\ensuremath{\underline{P}_{e}^{\mathrm{i}}\left({#1}\right)}}

\newcommand{\Wt}[1]{\ensuremath{\wt\left({#1}\right)}}
\newcommand{\Dist}[1]{\ensuremath{d\left({#1}\right)}}

\newcommand{\ppol}{\ensuremath{\overline{p}_{\scriptscriptstyle{\mathrm{TSB}}}}}
\newcommand{\psspb}
{\ensuremath{\underline{p}_{\scriptscriptstyle{\mathrm{SPB}}}}}
\newcommand{\pseg}{\ensuremath{\underline{p}_{\scriptscriptstyle{L_2}}}}
\newcommand{\pbub}[1]{\ensuremath{\overline{p}_{N}\left({#1}\right)}}
\newcommand{\pblb}[1]{\ensuremath{\underline{p}_{N}\left({#1}\right)}}

\newcommand{\Heaviside}[1]{\ensuremath{u\left({#1}\right)}}

\newcommand{\Nca}{\ensuremath{N_c^{\ast}}}
\newcommand{\Nc}{\ensuremath{N_c}}
\newcommand{\Ncset}{\ensuremath{\mathcal{N}}}

\newcommand{\mset}{\ensuremath{\mathcal{M}}}

\newcommand{\defeq}{\triangleq}

\newcommand{\Dham}[1]{\ensuremath{\dist\left({#1}\right)}}

\newcommand{\Deg}[1]{\ensuremath{\deg\left({#1}\right)}}
\newcommand{\Rank}[1]{\ensuremath{\rank\left({#1}\right)}}


==> env.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% env.tex                                                                      %
% created: Apr 14 2000, gs                                                     %
% last changed: Apr 14 2000, gs                                                %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

{\theoremstyle{break}
   \theorembodyfont{\rmfamily}
   \newtheorem{problem}{Problem}}

{\theoremstyle{break}
   \newtheorem{definition}{Definition}}

{\theoremstyle{plain}
   \newtheorem{theorem}{Theorem}}

{\theoremstyle{plain}
   \newtheorem{corollary}{Corollary}}

{\theoremstyle{plain}
   \newtheorem{lemma}{Lemma}}

